Evolutionary Algorithm and Multifactorial Evolutionary Algorithm on Clustered Shortest-Path Tree problem

In literature, Clustered Shortest-Path Tree Problem (CluSPT) is an NP-hard problem. Previous studies often search for an optimal solution in relatively large space. To enhance the performance of the search process, two approaches are proposed: the first approach seeks for solutions as a set of edges. From the original graph, we generate a new graph whose vertex set's cardinality is much smaller than that of the original one. Consequently, an effective Evolutionary Algorithm (EA) is proposed for solving CluSPT. The second approach looks for vertex-based solutions. The search space of the CluSPT is transformed into 2 nested search spaces (NSS). With every candidate in the high-level optimization, the search engine in the lower level will find a corresponding candidate to combine with it to create the best solution for CluSPT. Accordingly, Nested Local Search EA (N-LSEA) is introduced to search for the optimal solution on the NSS. When solving this model in lower level by N-LSEA, variety of similar tasks are handled. Thus, Multifactorial Evolutionary Algorithm applied in order to enhance the implicit genetic transfer across these optimizations. Proposed algorithms are conducted on a series of datasets and the obtained results demonstrate superior efficiency in comparison to previous scientific works.

==> Tables/Type1Large_EAM_RPD.tex <==
% Table generated by Excel2LaTeX from sheet 'BF-Avg-Time (2)'
\begin{table}[htbp]
  \centering
  \caption{Relative Percentage Differences Between Results obtained by AEM and GACSPT, N-LSEA, M-LSEA on Instances In Type 1 Large.}
    \begin{tabular}{|l|r|r|r|r|}
    \hline
    \multicolumn{1}{|c|}{\multirow{2}[4]{*}{\textbf{Instances}}} & \multicolumn{1}{c|}{\multirow{2}[4]{*}{\textbf{EAM}}} & \multicolumn{3}{c|}{\textbf{RPD(.)}} \\
	\cline{3-5}          &       & 
	\multicolumn{1}{c|}{\textbf{GACSPT}} & \multicolumn{1}{c|}{\textbf{M-LSEA}} & \multicolumn{1}{c|}{\textbf{N-LSEA}} \\
    \hline
    10a280 & 27925.2 & 0.21\% & 0.47\% & 0.48\% \\
    \hline
    10gil262 & 27637.5 & 0.12\% & 0.08\% & 0.12\% \\
    \hline
    10lin318 & 809750.0 & 0.02\% & 0.04\% & 0.04\% \\
    \hline
    10pcb442 & 741195.8 & 0.14\% & 0.08\% & 0.15\% \\
    \hline
    10pr439 & 1904690.2 & 0.05\% & 0.12\% & 0.14\% \\
    \hline
    150nrw1379 & 1261803.9 & 51.07\% & 67.45\% & 84.98\% \\
    \hline
    150pcb1173 & 1728190.8 & 37.43\% & 44.69\% & 56.27\% \\
    \hline
    150pr1002 & 6258631.9 & 50.47\% & 63.33\% & 78.83\% \\
    \hline
    150rat783 & 204410.4 & 34.65\% & 45.81\% & 58.61\% \\
    \hline
    150vm1084 & 7741281.1 & 42.46\% & 59.53\% & 74.91\% \\
    \hline
    25a280 & 29902.4 & 3.32\% & 12.04\% & 12.29\% \\
    \hline
    25gil262 & 30325.7 & 1.97\% & 9.21\% & 9.75\% \\
    \hline
    25lin318 & 584554.0 & 3.72\% & 10.98\% & 11.21\% \\
    \hline
    25pcb442 & 740892.6 & 3.02\% & 13.72\% & 14.48\% \\
    \hline
    25pr439 & 1511168.9 & 3.53\% & 12.31\% & 12.95\% \\
    \hline
    50a280 & 36266.9 & 8.98\% & 15.46\% & 20.47\% \\
    \hline
    50gil262 & 26523.3 & 9.70\% & 19.06\% & 24.88\% \\
    \hline
    50lin318 & 688724.6 & 6.36\% & 13.98\% & 17.97\% \\
    \hline
    50nrw1379 & 1831566.9 & 6.47\% & 12.54\% & 15.92\% \\
    \hline
    50pcb1173 & 1108183.8 & 17.05\% & 27.80\% & 35.49\% \\
    \hline
    50pcb442 & 910478.7 & 8.08\% & 15.80\% & 19.91\% \\
    \hline
    50pr1002 & 5243008.7 & 13.85\% & 24.70\% & 32.11\% \\
    \hline
    50pr439 & 2152986.6 & 8.14\% & 14.53\% & 19.27\% \\
    \hline
    \end{tabular}%
  \label{tab:Results_Type1Large_RPD}%
\end{table}%


==> Tables/Type1Small_EAM_RPD.tex <==
% Table generated by Excel2LaTeX from sheet 'BF-Avg-Time (2)'
\begin{table}[htbp]
  \centering
  \caption{Relative Percentage Differences Between Results Obtained by AEM and GACSPT, N-LSEA, M-LSEA on Instances In Type 1 Small.}
    \begin{tabular}{|l|r|r|r|r|}
    \hline
    \multicolumn{1}{|c|}{\multirow{2}[4]{*}{\textbf{Instances}}} & \multicolumn{1}{c|}{\textbf{EAM}} & \multicolumn{3}{c|}{\textbf{RPD(.)}} \\
	\cline{2-5}          &       & \multicolumn{1}{c|}{\textbf{GACSPT}} & \multicolumn{1}{c|}{\textbf{M-LSEA}} & \multicolumn{1}{c|}{\textbf{N-LSEA}} \\
    \hline
    10berlin52 & 43724.1 & 0.00\% & 0.20\% & 0.33\% \\
    \hline
    10eil51 & 1713.2 & 0.14\% & 0.25\% & 0.34\% \\
    \hline
    10eil76 & 2203.3 & 0.23\% & 0.21\% & 0.37\% \\
    \hline
    10kroB100 & 140522.2 & 0.08\% & 0.09\% & 0.08\% \\
    \hline
    10pr76 & 522213.8 & 0.04\% & 0.21\% & 0.37\% \\
    \hline
    10rat99 & 7520.2 & 0.09\% & 0.11\% & 0.17\% \\
    \hline
    10st70 & 3095.2 & 0.16\% & 0.06\% & 0.13\% \\
    \hline
    15berlin52 & 26312.0 & 0.22\% & 3.47\% & 4.88\% \\
    \hline
    15eil51 & 1306.4 & 0.44\% & 4.12\% & 3.92\% \\
    \hline
    15eil76 & 2909.1 & 0.26\% & 2.13\% & 2.78\% \\
    \hline
    15pr76 & 704600.6 & 0.45\% & 3.06\% & 2.41\% \\
    \hline
    15st70 & 4120.1 & 0.58\% & 1.84\% & 2.01\% \\
    \hline
    25eil101 & 4679.0 & 2.03\% & 8.93\% & 10.08\% \\
    \hline
    25kroA100 & 147195.0 & 2.15\% & 8.88\% & 9.09\% \\
    \hline
    25lin105 & 97944.7 & 2.38\% & 8.50\% & 8.83\% \\
    \hline
    25rat99 & 6841.5 & 3.18\% & 11.87\% & 12.12\% \\
    \hline
    50eil101 & 3825.3 & 7.88\% & 16.30\% & 20.67\% \\
    \hline
    50kroA100 & 159647.2 & 8.29\% & 16.35\% & 22.07\% \\
    \hline
    50kroB100 & 133104.5 & 10.39\% & 20.38\% & 29.56\% \\
    \hline
    50lin105 & 145829.1 & 3.68\% & 9.08\% & 14.94\% \\
    \hline
    50rat99 & 8007.4 & 10.18\% & 16.40\% & 24.26\% \\
    \hline
    5berlin52 & 22746.4 & 0.00\% & 0.00\% & 0.00\% \\
    \hline
    5eil51 & 1769.4 & 0.00\% & 0.00\% & 0.00\% \\
    \hline
    5eil76 & 2630.8 & 0.00\% & 0.00\% & 0.00\% \\
    \hline
    5pr76 & 585008.0 & 0.00\% & 0.00\% & 0.00\% \\
    \hline
    5st70 & 4520.1 & 0.00\% & 0.00\% & 0.00\% \\
    \hline
    75lin105 & 156944.7 & 5.17\% & 14.07\% & 22.31\% \\
    \hline
    \end{tabular}%
  \label{tab:Results_Type1Small_RPD}%
\end{table}%


==> Tables/Type2-1.tex <==
\begin{table*}[htbp]
  \centering
  \caption{Results Obtained By GACSPT, N-LSEA, M-LSEA and EAM on Instances In Type 2}
  \begin{tabular}{|l|l|r|r|r|l|r|r|r|r|r|}
	    \hline
	    \multicolumn{1}{|c|}{\multirow{2}[4]{*}{\textbf{Instance}}} & 
	    \multicolumn{2}{p{11.5em}|}{\textbf{GACSPT}} & 
	    \multicolumn{2}{p{11.22em}|}{\textbf{M-LSEA}} & 
	    \multicolumn{2}{p{11.5em}|}{\textbf{N-LSEA}} & 
	    \multicolumn{1}{c|}{\multirow{2}[4]{*}{\textbf{EAM}}} & 
	    \multicolumn{3}{c|}{\textbf{RPD(.)}} \\
	    
		\cline{2-7}
		\cline{9-11}          & 
		\multicolumn{1}{c|}{\textbf{Min}} & 
		\multicolumn{1}{c|}{\textbf{Mean}} & 
		\multicolumn{1}{c|}{\textbf{Min}} & 
		\multicolumn{1}{c|}{\textbf{Mean}} & 
		\multicolumn{1}{c|}{\textbf{Min}} & 
		\multicolumn{1}{c|}{\textbf{Mean}} &       & 
		\multicolumn{1}{p{3.5em}|}{\textbf{GACSPT}} & 
		\multicolumn{1}{p{2em}|}{\textbf{M-LSEA}} & 
		\multicolumn{1}{p{2em}|}{\textbf{N-LSEA}} \\
	    \hline
	    10C1k.0 & 603982229.6 & 604675739.3 & 603896769.1 & 604075680.5 & 603896769.1 & 604205712.3 & 603896769.1 & 0.13\% & 0.03\% & 0.05\% \\
	    \hline
	    10C1k.1 & 555719300.5 & 556214402.2 & 555519829.5 & 555601193 & 555519829.5 & 555655243.8 & 555519829.5 & 0.13\% & 0.01\% & 0.02\% \\
	    \hline
	    10C1k.2 & 740604616.4 & 741022869.8 & 740549053.6 & 740684380.1 & 740549053.5 & 740844678.6 & 740549053.6 & 0.06\% & 0.02\% & 0.04\% \\
	    \hline
	    10C1k.3 & 594441714.7 & 594586353.6 & 594412757.2 & 594496659.8 & 594412757.2 & 594664542.2 & 594412757.2 & 0.03\% & 0.01\% & 0.04\% \\
	    \hline
	    10C1k.4 & 533230914.9 & 533679392.5 & 533153746.9 & 533199581.9 & 533153746.9 & 533241310.4 & 533153746.9 & 0.10\% & 0.01\% & 0.02\% \\
	    \hline
	    10C1k.5 & 582566421.6 & 582865515.5 & 582557709.0 & 582706836.6 & 582557709.0 & 582785381.2 & 582557709.0 & 0.05\% & 0.03\% & 0.04\% \\
	    \hline
	    10C1k.6 & 581100882.1 & 582046361.4 & 580986510.1 & 581062186.1 & 580986510.0 & 581113261.8 & 580986510.1 & 0.18\% & 0.01\% & 0.02\% \\
	    \hline
	    10C1k.7 & 343334932.7 & 343819864.2 & 343312412.6 & 343395225.6 & 343312412.6 & 343503363 & 343312412.6 & 0.15\% & 0.02\% & 0.06\% \\
	    \hline
	    10C1k.8 & 564506471.2 & 564723479.2 & 564496866.9 & 564663214.5 & 564496866.8 & 564804840.7 & 564496866.9 & 0.04\% & 0.03\% & 0.05\% \\
	    \hline
	    10C1k.9 & 423567170.4 & 423891849.3 & 423562402.5 & 423582414.7 & 423562402.5 & 423618392.5 & 423562402.5 & 0.08\% & 0.00\% & 0.01\% \\
	    \hline
    \end{tabular}%
  	\label{tab:Results_Type2}%
\end{table*}%


==> Tables/Type2.tex <==
\begin{table*}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|l|l|r|r|r|l|r|r|r|r|r|}
    \hline
    \multicolumn{1}{|c|}{\multirow{2}[4]{*}{\textbf{Instances}}} & 
    \multicolumn{2}{p{11.5em}|}{\textbf{GACSPT}} & 
    \multicolumn{2}{p{11.22em}|}{\textbf{M-LSEA}} & 
    \multicolumn{2}{p{11.5em}|}{\textbf{N-LSEA}} & 
    \multicolumn{1}{c|}{\multirow{2}[4]{*}{\textbf{EAM}}} & 
    \multicolumn{3}{c|}{\textbf{RPD(.)}} \\
    
	\cline{2-7}
	\cline{9-11}          & 
	\multicolumn{1}{c|}{\textbf{Min}} & 
	\multicolumn{1}{c|}{\textbf{Mean}} & 
	\multicolumn{1}{c|}{\textbf{Min}} & 
	\multicolumn{1}{c|}{\textbf{Mean}} & 
	\multicolumn{1}{c|}{\textbf{Min}} & 
	\multicolumn{1}{c|}{\textbf{Mean}} &       & 
	\multicolumn{1}{c|}{\textbf{GACSPT}} & 
	\multicolumn{1}{c|}{\textbf{M-LSEA}} & 
	\multicolumn{1}{c|}{\textbf{N-LSEA}} \\
    \hline
    10C1k.0 & 603982229.65 & 604675739.3 & 603896769.1 & 604075680.5 & 603896769.13 & 604205712.3 & 603896769.1 & 0.13\% & 0.03\% & 0.05\% \\
    \hline
    10C1k.1 & 555719300.53 & 556214402.2 & 555519829.5 & 555601193 & 555519829.51 & 555655243.8 & 555519829.5 & 0.13\% & 0.01\% & 0.02\% \\
    \hline
    10C1k.2 & 740604616.46 & 741022869.8 & 740549053.6 & 740684380.1 & 740549053.58 & 740844678.6 & 740549053.6 & 0.06\% & 0.02\% & 0.04\% \\
    \hline
    10C1k.3 & 594441714.72 & 594586353.6 & 594412757.2 & 594496659.8 & 594412757.23 & 594664542.2 & 594412757.2 & 0.03\% & 0.01\% & 0.04\% \\
    \hline
    10C1k.4 & 533230914.94 & 533679392.5 & 533153746.9 & 533199581.9 & 533153746.94 & 533241310.4 & 533153746.9 & 0.10\% & 0.01\% & 0.02\% \\
    \hline
    10C1k.5 & 582566421.65 & 582865515.5 & 582557709 & 582706836.6 & 582557709.03 & 582785381.2 & 582557709.0 & 0.05\% & 0.03\% & 0.04\% \\
    \hline
    10C1k.6 & 581100882.13 & 582046361.4 & 580986510.1 & 581062186.1 & 580986510.08 & 581113261.8 & 580986510.1 & 0.18\% & 0.01\% & 0.02\% \\
    \hline
    10C1k.7 & 343334932.78 & 343819864.2 & 343312412.6 & 343395225.6 & \multicolumn{1}{r|}{343312412.6} & 343503363 & 343312412.6 & 0.15\% & 0.02\% & 0.06\% \\
    \hline
    10C1k.8 & 564506471.22 & 564723479.2 & 564496866.9 & 564663214.5 & 564496866.87 & 564804840.7 & 564496866.9 & 0.04\% & 0.03\% & 0.05\% \\
    \hline
    10C1k.9 & 423567170.45 & 423891849.3 & 423562402.5 & 423582414.7 & 423562402.54 & 423618392.5 & 423562402.5 & 0.08\% & 0.00\% & 0.01\% \\
    \hline
    \end{tabular}%
  \label{tab:addlabel}%
\end{table*}%


==> Tables/Type3.tex <==
% Table generated by Excel2LaTeX from sheet 'Type 3'
\begin{table*}[htbp]
  \centering
  \caption{Results Obtained By GACSPT, N-LSEA, M-LSEA and EAM on Instances in Type 3}
    \begin{tabular}{|l|l|r|r|r|r|r|r|r|r|r|}
    \hline
    \multicolumn{1}{|c|}{\multirow{2}[4]{*}{\textbf{Instance}}}& \multicolumn{2}{p{8em}|}{\textbf{GACSPT}} & \multicolumn{2}{p{8.11em}|}{\textbf{M-LSEA}} & \multicolumn{2}{p{8.11em}|}{\textbf{N-LSEA}} & \multicolumn{1}{c|}{\multirow{2}[4]{*}{\textbf{EAM}}} & \multicolumn{3}{c|}{\textbf{RPD(.)}} \\
    
	\cline{2-7}\cline{9-11}          & 
	\multicolumn{1}{c|}{\textbf{Min}} & 
	\multicolumn{1}{c|}{\textbf{Mean}} & 
	\multicolumn{1}{c|}{\textbf{Min}} & 
	\multicolumn{1}{c|}{\textbf{Mean}} & 
	\multicolumn{1}{c|}{\textbf{Min}} & 
	\multicolumn{1}{c|}{\textbf{Mean}} &       & \multicolumn{1}{c|}{\textbf{GACSPT}} & \multicolumn{1}{c|}{\textbf{M-LSEA}} & \multicolumn{1}{c|}{\textbf{N-LSEA}} \\
    \hline
    6i300 & 19264.45 & 19278.27 & 19264.45 & 19265.02 & 19264.45 & 19264.51 & 19264.5 & 0.07\% & 0.00\% & 0.00\% \\
    \hline
    6i350 & 21217.20 & 21236.25 & 21217.2 & 21217.2 & 21217.2 & 21217.2 & 21217.2 & 0.09\% & 0.00\% & 0.00\% \\
    \hline
    6i400 & 29348.22 & 29350.07 & 29348.22 & 29348.22 & 29348.22 & 29348.39 & 29348.2 & 0.01\% & 0.00\% & 0.00\% \\
    \hline
    6i450 & 35681.53 & 35684.23 & 35681.53 & 35682.52 & 35681.53 & 35682.82 & 35681.5 & 0.01\% & 0.00\% & 0.00\% \\
    \hline
    6i500 & 37510.09 & 37516.01 & 37510.09 & 37510.71 & 37510.09 & 37510.58 & 37510.1 & 0.02\% & 0.00\% & 0.00\% \\
    \hline
    \end{tabular}%
  \label{tab:Results_Type3}%
\end{table*}%


==> Tables/Type4.tex <==
% Table generated by Excel2LaTeX from sheet 'Type 4'
\begin{table*}[htbp]
  \centering
  \caption{Results Obtained By GACSPT, N-LSEA, M-LSEA and EAM on Instances in Type 4}
    \begin{tabular}{|l|l|l|r|r|l|r|r|r|r|r|}
    \hline
    \multicolumn{1}{|c|}{\multirow{2}[4]{*}{\textbf{Instances}}} & \multicolumn{2}{p{8.78em}|}{\textbf{GACSPT}} & \multicolumn{2}{p{9.22em}|}{\textbf{M-LSEA}} & \multicolumn{2}{p{9em}|}{\textbf{N-LSEA}} & \multicolumn{1}{c|}{\multirow{2}[4]{*}{\textbf{EAM}}} & \multicolumn{3}{c|}{\textbf{RPD(.)}} \\
\cline{2-7}\cline{9-11}          & \multicolumn{1}{c|}{\textbf{Min}} & \multicolumn{1}{c|}{\textbf{Mean}} & \multicolumn{1}{c|}{\textbf{Min}} & \multicolumn{1}{c|}{\textbf{Mean}} & \multicolumn{1}{c|}{\textbf{Min}} & \multicolumn{1}{c|}{\textbf{Mean}} &       & \multicolumn{1}{c|}{\textbf{GACSPT}} & \multicolumn{1}{c|}{\textbf{M-LSEA}} & \multicolumn{1}{c|}{\textbf{N-LSEA}} \\
    \hline
    4i200a & 97959.60 & 98392.18 & 97959.6 & 97959.6 & 97959.60 & 97959.6 & 97959.6 & 0.44\% & 0.00\% & 0.00\% \\
    \hline
    4i200h & 87675.31 & 87778.94 & 87675.31 & 87675.31 & 87675.31 & 87675.31 & 87675.3 & 0.12\% & 0.00\% & 0.00\% \\
    \hline
    4i200x1 & 123669.70 & 123751.30 & 123669.7 & 123669.7 & 123669.70 & 123669.7 & 123669.7 & 0.07\% & 0.00\% & 0.00\% \\
    \hline
    4i200x2 & 114012.32 & 114060.34 & 114012.33 & 114012.33 & 114012.33 & 114012.33 & 114012.3 & 0.04\% & 0.00\% & 0.00\% \\
    \hline
    4i200z & 131683.50 & 131703.35 & 131683.5 & 131683.5 & 131683.50 & 131683.5 & 131683.5 & 0.02\% & 0.00\% & 0.00\% \\
    \hline
    4i400a & 214115.33 & 219283.54 & 214115.33 & 214115.33 & 214115.33 & 214115.33 & 214115.3 & 2.41\% & 0.00\% & 0.00\% \\
    \hline
    4i400h & 256200.51 & 256272.73 & 256200.51 & 256200.51 & 256200.51 & 256200.51 & 256200.5 & 0.03\% & 0.00\% & 0.00\% \\
    \hline
    4i400x1 & 188196.75 & 188408.00 & 188196.75 & 188196.75 & 188196.75 & 188196.75 & 188196.7 & 0.11\% & 0.00\% & 0.00\% \\
    \hline
    4i400x2 & 159254.77 & 160086.56 & 159254.77 & 159254.77 & 159254.77 & 159254.77 & 159254.8 & 0.52\% & 0.00\% & 0.00\% \\
    \hline
    4i400z & 221423.87 & 221592.66 & 221423.87 & 221423.87 & 221423.87 & 221423.87 & 221423.9 & 0.08\% & 0.00\% & 0.00\% \\
    \hline
    \end{tabular}%
  \label{tab:Results_Type4}%
\end{table*}%


==> Tables/Type5Large.tex <==
% Table generated by Excel2LaTeX from sheet 'Type 5 Large'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|l|r|r|r|l|l|l|r|r|r|r|}
    \toprule
    \multicolumn{1}{|c|}{\multirow{2}[4]{*}{\textbf{Instances}}} & \multicolumn{2}{p{8.78em}|}{\textbf{GACSPT}} & \multicolumn{2}{p{9.22em}|}{\textbf{M-LSEA}} & \multicolumn{2}{p{9em}|}{\textbf{N-LSEA}} & \multicolumn{1}{c|}{\multirow{2}[4]{*}{\textbf{EAM}}} & \multicolumn{3}{c|}{\textbf{RPD(.)}} \\
\cmidrule{2-7}\cmidrule{9-11}          & \multicolumn{1}{c|}{\textbf{Min}} & \multicolumn{1}{c|}{\textbf{Mean}} & \multicolumn{1}{c|}{\textbf{Min}} & \multicolumn{1}{c|}{\textbf{Mean}} & \multicolumn{1}{c|}{\textbf{Min}} & \multicolumn{1}{c|}{\textbf{Mean}} &       & \multicolumn{1}{c|}{\textbf{GACSPT}} & \multicolumn{1}{c|}{\textbf{M-LSEA}} & \multicolumn{1}{c|}{\textbf{N-LSEA}} \\
    \midrule
    10i300-109 & 112681 & 112727 & 112681.01 & 112735.70 & 112681.01 & 112836.30 & 112681.0 & 0.04\% & 0.05\% & 0.14\% \\
    \midrule
    10i400-206 & 207521.7 & 207680.7 & 207521.67 & 207659.01 & 207521.67 & 207754.81 & 207521.7 & 0.08\% & 0.07\% & 0.11\% \\
    \midrule
    10i500-305 & 349676.6 & 349867.4 & 349675.23 & 349786.93 & 349675.23 & 349753.66 & 349675.2 & 0.05\% & 0.03\% & 0.02\% \\
    \midrule
    15i300-110 & 112096.7 & 112171.6 & 112393.02 & 113266.04 & 112577.15 & 113625.44 & 112096.7 & 0.07\% & 1.04\% & 1.36\% \\
    \midrule
    15i400-207 & 164117.8 & 164639.7 & 164271.74 & 165102.75 & 164526.87 & 165633.28 & 164117.8 & 0.32\% & 0.60\% & 0.92\% \\
    \midrule
    15i500-306 & 300742.1 & 301622.7 & 300893.24 & 301683.75 & 301089.56 & 302133.28 & 300734.1 & 0.30\% & 0.32\% & 0.47\% \\
    \midrule
    200i2000-606 & 1891129 & 2092509 & 2158246.4 & 2232903.72 & 2321654.05 & 2384238.86 & 1475366.9 & 41.83\% & 51.35\% & 61.60\% \\
    \midrule
    200i2500-710 & 1994094 & 2173749 & 2246518 & 2329187.47 & 2416473.95 & 2531295.77 & 1355011.2 & 60.42\% & 71.89\% & 86.81\% \\
    \midrule
    200i3000-805 & 2255767 & 2604482 & 2642053.6 & 2719577.33 & 2794935.18 & 2965489.65 & 1601021.2 & 62.68\% & 69.87\% & 85.22\% \\
    \midrule
    20i1000-408 & 468210.2 & 470540.7 & 474197.21 & 482607.73 & 476798.02 & 487856.23 & 467562.4 & 0.64\% & 3.22\% & 4.34\% \\
    \midrule
    20i1500-504 & 918090.9 & 922161.3 & 924919.69 & 931793.88 & 927655.95 & 938703.36 & 917765.2 & 0.48\% & 1.53\% & 2.28\% \\
    \midrule
    20i2000-602 & 1008231 & 1015629 & 1015882.6 & 1023325.80 & 1015831.51 & 1031809.51 & 1005626.8 & 0.99\% & 1.76\% & 2.60\% \\
    \midrule
    20i2500-706 & 1374111 & 1383760 & 1387986.6 & 1400171.31 & 1385462.62 & 1404259.33 & 1373157.9 & 0.77\% & 1.97\% & 2.26\% \\
    \midrule
    20i300-111 & 156347.7 & 158147.9 & 159748.89 & 164305.28 & 159485.61 & 165744.20 & 156347.7 & 1.15\% & 5.09\% & 6.01\% \\
    \midrule
    20i400-208 & 224023.8 & 225715.7 & 227590.91 & 234155.75 & 229122.45 & 236582.70 & 224012.5 & 0.76\% & 4.53\% & 5.61\% \\
    \midrule
    20i500-307 & 200332 & 202616.5 & 206036.85 & 212845.15 & 208000.23 & 214113.55 & 200328.7 & 1.14\% & 6.25\% & 6.88\% \\
    \midrule
    25i300-112 & 116282.2 & 118925.9 & 128229.1 & 134989.48 & 128379.81 & 136666.03 & 116193.6 & 2.35\% & 16.18\% & 17.62\% \\
    \midrule
    25i400-209 & 230554.8 & 235954.1 & 246371.98 & 254536.47 & 247441.72 & 255233.34 & 229913.6 & 2.63\% & 10.71\% & 11.01\% \\
    \midrule
    25i500-308 & 299528.8 & 302548.8 & 315899.96 & 323559.84 & 312869.24 & 326271.71 & 299498.2 & 1.02\% & 8.03\% & 8.94\% \\
    \midrule
    5i300-108 & 177185.9 & 177221.3 & 177185.93 & 177185.93 & 177185.93 & 177188.65 & 177185.9 & 0.02\% & 0.00\% & 0.00\% \\
    \midrule
    5i400-205 & 209389.8 & 209440.3 & 209389.82 & 209389.82 & 209389.82 & 209389.82 & 209389.8 & 0.02\% & 0.00\% & 0.00\% \\
    \midrule
    5i500-304 & 182024.7 & 182045.9 & 182024.03 & 182024.03 & 182024.03 & 182024.03 & 182024.0 & 0.01\% & 0.00\% & 0.00\% \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%


==> Tables/Type5Large_EAM_RPD.tex <==
% Table generated by Excel2LaTeX from sheet 'BF-Avg-Time (2)'
\begin{table}[htbp]
  \centering
  \caption{Relative Percentage Differences Between Results obtained by AEM and GACSPT, N-LSEA, M-LSEA on Instances In Type 5 Large}
    \begin{tabular}{|l|r|r|r|r|}
    \hline
    \multicolumn{1}{|c|}{\multirow{2}[4]{*}{\textbf{Instances}}} & \multicolumn{1}{c|}{\textbf{EAM}} & \multicolumn{3}{c|}{\textbf{RPD(.)}} \\
	\cline{2-5}          &       & 
	\multicolumn{1}{c|}{\textbf{GACSPT}} & \multicolumn{1}{c|}{\textbf{M-LSEA}} & \multicolumn{1}{c|}{\textbf{N-LSEA}} \\
    \hline
    10i300-109 & 112681.0 & 0.04\% & 0.05\% & 0.14\% \\
    \hline
    10i400-206 & 207521.7 & 0.08\% & 0.07\% & 0.11\% \\
    \hline
    10i500-305 & 349675.2 & 0.05\% & 0.03\% & 0.02\% \\
    \hline
    15i300-110 & 112096.7 & 0.07\% & 1.04\% & 1.36\% \\
    \hline
    15i400-207 & 164117.8 & 0.32\% & 0.60\% & 0.92\% \\
    \hline
    15i500-306 & 300734.1 & 0.30\% & 0.32\% & 0.47\% \\
    \hline
    200i2000-606 & 1475366.9 & 41.83\% & 51.35\% & 61.60\% \\
    \hline
    200i2500-710 & 1355011.2 & 60.42\% & 71.89\% & 86.81\% \\
    \hline
    200i3000-805 & 1601021.2 & 62.68\% & 69.87\% & 85.22\% \\
    \hline
    20i1000-408 & 467562.4 & 0.64\% & 3.22\% & 4.34\% \\
    \hline
    20i1500-504 & 917765.2 & 0.48\% & 1.53\% & 2.28\% \\
    \hline
    20i2000-602 & 1005626.8 & 0.99\% & 1.76\% & 2.60\% \\
    \hline
    20i2500-706 & 1373157.9 & 0.77\% & 1.97\% & 2.26\% \\
    \hline
    20i300-111 & 156347.7 & 1.15\% & 5.09\% & 6.01\% \\
    \hline
    20i400-208 & 224012.5 & 0.76\% & 4.53\% & 5.61\% \\
    \hline
    20i500-307 & 200328.7 & 1.14\% & 6.25\% & 6.88\% \\
    \hline
    25i300-112 & 116193.6 & 2.35\% & 16.18\% & 17.62\% \\
    \hline
    25i400-209 & 229913.6 & 2.63\% & 10.71\% & 11.01\% \\
    \hline
    25i500-308 & 299498.2 & 1.02\% & 8.03\% & 8.94\% \\
    \hline
    5i300-108 & 177185.9 & 0.02\% & 0.00\% & 0.00\% \\
    \hline
    5i400-205 & 209389.8 & 0.02\% & 0.00\% & 0.00\% \\
    \hline
    5i500-304 & 182024.0 & 0.01\% & 0.00\% & 0.00\% \\
    \hline
    \end{tabular}%
  \label{tab:Results_Type5Large_RPD}%
\end{table}%


==> Tables/Type6Large.tex <==
% Table generated by Excel2LaTeX from sheet 'Type 6 Large'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|l|r|r|r|r|l|r|r|r|r|r|}
    \toprule
    \multicolumn{1}{|c|}{\multirow{2}[4]{*}{\textbf{Instances}}} & \multicolumn{2}{p{8.78em}|}{\textbf{GACSPT}} & \multicolumn{2}{p{9.22em}|}{\textbf{M-LSEA}} & \multicolumn{2}{p{10em}|}{\textbf{N-LSEA}} & \multicolumn{1}{c|}{\multirow{2}[4]{*}{\textbf{EAM}}} & \multicolumn{3}{c|}{\textbf{RPD(.)}} \\
\cmidrule{2-7}\cmidrule{9-11}          & \multicolumn{1}{c|}{\textbf{Min}} & \multicolumn{1}{c|}{\textbf{Mean}} & \multicolumn{1}{c|}{\textbf{Min}} & \multicolumn{1}{c|}{\textbf{Mean}} & \multicolumn{1}{c|}{\textbf{Min}} & \multicolumn{1}{c|}{\textbf{Mean}} &       & \multicolumn{1}{c|}{\textbf{GACSPT}} & \multicolumn{1}{c|}{\textbf{M-LSEA}} & \multicolumn{1}{c|}{\textbf{N-LSEA}} \\
    \midrule
    100prb1173-10x10 & 1930392 & 2071547 & 2151529.8 & 2235551.1 & 2251880.51 & 2386566.3 & 1665836.8 & 24.35\% & 34.20\% & 43.27\% \\
    \midrule
    100rat783-10x10 & 174016.4 & 190040.4 & 207391.33 & 217450.72 & 221520.14 & 238693.4 & 135833.4 & 39.91\% & 60.09\% & 75.73\% \\
    \midrule
    10nrw1379-2x5 & 1318517 & 1323558 & 1317301.4 & 1317826 & 1317301.43 & 1317923.3 & 1317301.4 & 0.47\% & 0.04\% & 0.05\% \\
    \midrule
    12nrw1379-2x6 & 1243090 & 1257144 & 1239386 & 1241102.7 & 1239386.02 & 1241903.9 & 1239386.0 & 1.43\% & 0.14\% & 0.20\% \\
    \midrule
    12nrw1379-3x4 & 1486829 & 1490375 & 1486754.7 & 1487880.3 & 1486729.54 & 1488527.1 & 1486648.6 & 0.25\% & 0.08\% & 0.13\% \\
    \midrule
    144pcb1173-12x12 & 1650024 & 1825097 & 2004711.3 & 2058787.4 & 2104321.22 & 2252633.3 & 1185361.4 & 53.97\% & 73.68\% & 90.04\% \\
    \midrule
    144rat783-12x12 & 282192 & 299267.7 & 302651.85 & 315549.29 & 327006.74 & 342296.81 & 225297.7 & 32.83\% & 40.06\% & 51.93\% \\
    \midrule
    18pr439-3x6 & 1472084 & 1480688 & 1495669.1 & 1526029.9 & 1499814.23 & 1527240.3 & 1471788.7 & 0.60\% & 3.69\% & 3.77\% \\
    \midrule
    20pr439-4x5 & 1978155 & 1993787 & 2004829.9 & 2035944.8 & 2010075.14 & 2044879.2 & 1978001.3 & 0.80\% & 2.93\% & 3.38\% \\
    \midrule
    25a280-5x5 & 41712.96 & 42362.86 & 43327.73 & 45577.6 & 43998.66 & 45831.18 & 41690.3 & 1.61\% & 9.32\% & 9.93\% \\
    \midrule
    25gil262-5x5 & 30711.92 & 31178.8 & 32847.72 & 33760.2 & 32995.81 & 34108.01 & 30649.5 & 1.73\% & 10.15\% & 11.28\% \\
    \midrule
    25lin318-5x5 & 715116.5 & 726620.3 & 764621 & 781227.16 & 758213.67 & 784246.32 & 715009.6 & 1.62\% & 9.26\% & 9.68\% \\
    \midrule
    25pcb442-5x5 & 740883.3 & 760869.8 & 808312.94 & 838117.16 & 822598.57 & 844904.84 & 740883.3 & 2.70\% & 13.12\% & 14.04\% \\
    \midrule
    36pcb442-6x6 & 863522.7 & 900900.4 & 935979.17 & 974970.94 & 964538.74 & 994331.83 & 860978.2 & 4.64\% & 13.24\% & 15.49\% \\
    \midrule
    36pr1002-6x6 & 5847062 & 6120589 & 6593220 & 6841454 & 6770556.51 & 6981861.9 & 5800806.4 & 5.51\% & 17.94\% & 20.36\% \\
    \midrule
    42a280-6x7 & 44514.51 & 46047.71 & 47212.15 & 48859.29 & 48525.94 & 49654.47 & 43896.8 & 4.90\% & 11.30\% & 13.12\% \\
    \midrule
    42pr1002-6x7 & 7189930 & 7479862 & 7801486.9 & 8111203.7 & 7998019.22 & 8295123.1 & 6974749.7 & 7.24\% & 16.29\% & 18.93\% \\
    \midrule
    49gil262-7x7 & 33156.15 & 34426.24 & 35565.37 & 36922.32 & 36850.85 & 38392.92 & 32130.5 & 7.15\% & 14.91\% & 19.49\% \\
    \midrule
    49lin318-7x7 & 586512.4 & 625703.5 & 651961.02 & 670013.34 & 676284.09 & 706475.81 & 569746.3 & 9.82\% & 17.60\% & 24.00\% \\
    \midrule
    49pcb1173-7x7 & 1436187 & 1532484 & 1605570.7 & 1682327.7 & 1673411.27 & 1754706.1 & 1379851.3 & 11.06\% & 21.92\% & 27.17\% \\
    \midrule
    49pr1002-7x7 & 7329741 & 7626061 & 7699692.7 & 7993580.3 & 8003380.58 & 8290583.7 & 6894864.5 & 10.60\% & 15.94\% & 20.24\% \\
    \midrule
    49rat783-7x7 & 236409.1 & 245741.3 & 259615.92 & 263980.93 & 264175.08 & 271575.3 & 231140.8 & 6.32\% & 14.21\% & 17.49\% \\
    \midrule
    49vm1084-7x7 & 7712747 & 8184598 & 8583738.4 & 8926994.6 & 8857519.97 & 9294158.2 & 7466097.6 & 9.62\% & 19.57\% & 24.48\% \\
    \midrule
    72vm1084-8x9 & 7900284 & 8559406 & 9072194.5 & 9359547.1 & 9644992.00 & 9961561 & 7357094.5 & 16.34\% & 27.22\% & 35.40\% \\
    \midrule
    81vm1084-9x9 & 9010431 & 9762762 & 10027522 & 10365002 & 10559177.39 & 10932291 & 8286234.5 & 17.82\% & 25.09\% & 31.93\% \\
    \midrule
    9a280-3x3 & 28947.46 & 29041.77 & 28947.46 & 28973.29 & 28947.46 & 28966.02 & 28947.5 & 0.33\% & 0.09\% & 0.06\% \\
    \midrule
    9gil262-3x3 & 20935.93 & 20955.77 & 20935.93 & 20956.19 & 20935.93 & 20952.44 & 20935.9 & 0.09\% & 0.10\% & 0.08\% \\
    \midrule
    9lin318-3x3 & 716850.2 & 717151.1 & 717040.95 & 717586.28 & 717040.95 & 717920.49 & 716850.2 & 0.04\% & 0.10\% & 0.15\% \\
    \midrule
    9pcb442-3x3 & 760238.3 & 763669.9 & 760238.26 & 760536.79 & 760238.26 & 760939.93 & 760238.3 & 0.45\% & 0.04\% & 0.09\% \\
    \midrule
    9pr439-3x3 & 1800754 & 1805313 & 1800753.9 & 1803300.6 & 1800753.86 & 1802816.7 & 1800753.9 & 0.25\% & 0.14\% & 0.11\% \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%


==> Tables/Type6Large_EAM_RPD.tex <==
% Table generated by Excel2LaTeX from sheet 'BF-Avg-Time (2)'
\begin{table}[htbp]
  \centering
  \caption{Relative Percentage Differences Between Results obtained by AEM and GACSPT, N-LSEA, M-LSEA on Instances In Type 6 Large}
    \begin{tabular}{|l|r|r|r|r|}
    \hline
    \multicolumn{1}{|c|}{\multirow{2}[4]{*}{\textbf{Instances}}} & \multicolumn{1}{c|}{\textbf{EAM}} & \multicolumn{3}{c|}{\textbf{RPD(.)}} \\
\cline{2-5}          &       & \multicolumn{1}{c|}{\textbf{GACSPT}} & \multicolumn{1}{c|}{\textbf{M-LSEA}} & \multicolumn{1}{c|}{\textbf{N-LSEA}} \\
    \hline
    100prb1173-10x10 & 1665836.8 & 24.35\% & 34.20\% & 43.27\% \\
    \hline
    100rat783-10x10 & 135833.4 & 39.91\% & 60.09\% & 75.73\% \\
    \hline
    10nrw1379-2x5 & 1317301.4 & 0.47\% & 0.04\% & 0.05\% \\
    \hline
    12nrw1379-2x6 & 1239386.0 & 1.43\% & 0.14\% & 0.20\% \\
    \hline
    12nrw1379-3x4 & 1486648.6 & 0.25\% & 0.08\% & 0.13\% \\
    \hline
    144pcb1173-12x12 & 1185361.4 & 53.97\% & 73.68\% & 90.04\% \\
    \hline
    144rat783-12x12 & 225297.7 & 32.83\% & 40.06\% & 51.93\% \\
    \hline
    18pr439-3x6 & 1471788.7 & 0.60\% & 3.69\% & 3.77\% \\
    \hline
    20pr439-4x5 & 1978001.3 & 0.80\% & 2.93\% & 3.38\% \\
    \hline
    25a280-5x5 & 41690.3 & 1.61\% & 9.32\% & 9.93\% \\
    \hline
    25gil262-5x5 & 30649.5 & 1.73\% & 10.15\% & 11.28\% \\
    \hline
    25lin318-5x5 & 715009.6 & 1.62\% & 9.26\% & 9.68\% \\
    \hline
    25pcb442-5x5 & 740883.3 & 2.70\% & 13.12\% & 14.04\% \\
    \hline
    36pcb442-6x6 & 860978.2 & 4.64\% & 13.24\% & 15.49\% \\
    \hline
    36pr1002-6x6 & 5800806.4 & 5.51\% & 17.94\% & 20.36\% \\
    \hline
    42a280-6x7 & 43896.8 & 4.90\% & 11.30\% & 13.12\% \\
    \hline
    42pr1002-6x7 & 6974749.7 & 7.24\% & 16.29\% & 18.93\% \\
    \hline
    49gil262-7x7 & 32130.5 & 7.15\% & 14.91\% & 19.49\% \\
    \hline
    49lin318-7x7 & 569746.3 & 9.82\% & 17.60\% & 24.00\% \\
    \hline
    49pcb1173-7x7 & 1379851.3 & 11.06\% & 21.92\% & 27.17\% \\
    \hline
    49pr1002-7x7 & 6894864.5 & 10.60\% & 15.94\% & 20.24\% \\
    \hline
    49rat783-7x7 & 231140.8 & 6.32\% & 14.21\% & 17.49\% \\
    \hline
    49vm1084-7x7 & 7466097.6 & 9.62\% & 19.57\% & 24.48\% \\
    \hline
    72vm1084-8x9 & 7357094.5 & 16.34\% & 27.22\% & 35.40\% \\
    \hline
    81vm1084-9x9 & 8286234.5 & 17.82\% & 25.09\% & 31.93\% \\
    \hline
    9a280-3x3 & 28947.5 & 0.33\% & 0.09\% & 0.06\% \\
    \hline
    9gil262-3x3 & 20935.9 & 0.09\% & 0.10\% & 0.08\% \\
    \hline
    9lin318-3x3 & 716850.2 & 0.04\% & 0.10\% & 0.15\% \\
    \hline
    9pcb442-3x3 & 760238.3 & 0.45\% & 0.04\% & 0.09\% \\
    \hline
    9pr439-3x3 & 1800753.9 & 0.25\% & 0.14\% & 0.11\% \\
    \hline
    \end{tabular}%
  \label{tab:Results_Type6Large_RPD}%
\end{table}%


==> sec_metric.tex <==
In this section, we investigate \gls{cluspt} on metric graph. A metric graph is a complete graph with the edge length satisfying the triangle inequality, i.e., $w(x, y) \leq w(x, z) + w(z, y)$ for $x, y, z \in V$. The definition of metric \gls{cluspt} is given as  follow:

\textbf{Input:} Given an metric graph $G = (V, E, w)$ whose set vertex is divided into $k$ disjointed clusters $C = \left\{C_1, C_2,\ldots, C_k\right\}$. $G$ has a root, denoted by $r$. Without loss of generality, assuming that $r \in C_1$.\\

\textbf{Output:} A clustered spanning tree $T$ of graph $G$. \\

\textbf{Objective:} Minimize $\displaystyle Cost = \sum\limits_{v \in V} d(r, v)$ \\

Based on the special properties of metric graph, we design an exact algorithm for metric \gls{cluspt} by constructing a two-level star-like graph. A star is a tree which at most one vertex is internal, and the rest are leaves. \\

\textbf{Theorem 1}: if $T$ is an optimal solution of metric \gls{cluspt}, each local tree of $T$  is a star. \\
\begin{proof}
	According to proposition~\ref{pro:1}, each local tree of $T$ is a shortest path tree rooted at vertex $v$. Because of the completion and triangle inequality of metric graph $G$, the shortest path from any other vertex $v$ to $u$ includes a unique edge connecting $u$ and $v$. Therefore, a shortest path tree rooted at vertex $v$ of a metric graph is a star with the center is $v$, or each local tree of $T$ is a star.
\end{proof}

\textbf{Theorem 2}: if $T$ is an optimal solution of metric \gls{cluspt}, each inter-cluster edge in $T$ shall connect one root of local tree and the root $r$ of graph $G$.
\begin{proof}
	Consider a local tree in $T$ which is denoted as $S$. Assuming that the root of local tree $S$ is $v$. The unique path from the root $r$ to any vertex in $S$ must pass through $v$, then total cost which the local tree $S$ contributes to the objective function of $T$ is: 
	\begin{equation}
	    \displaystyle \sum\limits_{u \in S} d(u, r) = \sum\limits_{u \in S} d(u, v) + |S| \times d(v, r)\label{eq:lema2}
	\end{equation}
	Based on equation \eqref{eq:lema2}, $T$ is the optimal solution iff $d(v, r)$ is the shortest path distance between $v$ and $r$. And this context only happens when connecting $v$ and $r$ by the edge between those two vertices in the given graph $G$ because $G$ is a metric graph. Therefore, each inter-cluster edge in $T$ connect one root of local tree and the root $r$.
\end{proof}

\indent Based on Theorem 1 and Theorem  2, an optimal solution  for metric \gls{cluspt} is a clustered spanning tree which satisfying:\\
- Each local tree of is a star.\\
- Each inter-cluster edge is the edge which connects the root of a local tree of  and the root of given graph .\\
An illustration of this optimal solution is given by Figure~\ref{fig:fig_03}.

\renewcommand{\scalefigure}{0.3}
\begin{figure}[htbp]
  \centerline{\includegraphics[scale=\scalefigure]{images/3.png}}
  \caption{A sample of the optimal solution for metric \glsentrytext{cluspt}.}
  \label{fig_03}
\end{figure}

Based on the above inference,  we design an exact algorithm to solve metric \gls{cluspt}. This algorithm is denoted as \mbox{EAM} and shall build an optimal clustered spanning tree  as followed: \\
- The local tree of $T$ which is induced by cluster $C_1$ is a star whose center is $r$. \\
- For each cluster $C_i, (2 \leq i \leq k)$, the local tree of $T$ which is induced by cluster $C_i$ is a star whose center is $r_i$, satisfying $r_i \in C_i$  and $\displaystyle r_i = argmin\left\{f(v) | v \in C_i\right\}$ which: $\displaystyle f(v) = w(r, v) + \sum\limits_{u \in C_i} w(u, v)$ \\
$w(x, y)$ is the length edge between $x$ and $y$ in the given graph $G$. After building the local tree of cluster $C_i$, the edge between $r_i$ and $r$ is chosen as an inter-cluster edge in $T$, or $E(T) = E(T) \cup \left\{r_i, r\right\}$. \\
Algorithm~\ref{alg:EAM} presents those steps.

\begin{algorithm}[htbp]
	\KwIn{$G = (V, E)$, $G$ is a metric graph, $C = \left\{C_1, C_2,\ldots, C_k\right\}$, root $r$}
	\KwOut{\gls{cluspt} $T$ of $G$ and $C$} 
	\BlankLine
	\Begin
	{
		$T_1, T_2, \ldots, T_k \leftarrow$ All local trees of $T$\;
		$r_1, r_2, \ldots, r_k \leftarrow$ Roots of local trees.\;
		$r_1$ = $r$\;
		$V(T_1) = \left\{v, v \in C_1\right\}$\;
		$E(T_1) = \left\{(r_1, v), v \in C_1\right\}$\;
		\ForEach{$i \in \left\{2 \ldots k\right\}$}
		{
			$\displaystyle r_i = argmin\left\{f(v) | v \in C_i\right\}$ which: $\displaystyle f(v) = w(r, v) + \sum\limits_{u \in C_i} w(u, v)$ \;
			$V(T_i) = \left\{v, v \in C_i\right\}$\;
			$E(T_i) = \left\{(r_i, v), v \in C_i\right\}$\;
		}
	}
	\caption{EAM}
	\label{alg:EAM}
\end{algorithm}

